CSGaussian: Progressive Rate-Distortion Compression and Segmentation for 3D Gaussian Splatting

We present the first unified framework for rate-distortion-optimized compression and segmentation of 3D Gaussian Splatting (3DGS). While 3DGS has proven effective for both real-time rendering and semantic scene understanding, prior works have largely treated these tasks independently, leaving their joint consideration unexplored. Inspired by recent advances in rate-distortion-optimized 3DGS compression, this work integrates semantic learning into the compression pipeline to support decoder-side applications--such as scene editing and manipulation--that extend beyond traditional scene reconstruction and view synthesis. Our scheme features a lightweight implicit neural representation-based hyperprior, enabling efficient entropy coding of both color and semantic attributes while avoiding costly grid-based hyperprior as seen in many prior works. To facilitate compression and segmentation, we further develop compression-guided segmentation learning, consisting of quantization-aware training to enhance feature separability and a quality-aware weighting mechanism to suppress unreliable Gaussian primitives. Extensive experiments on the LERF and 3D-OVS datasets demonstrate that our approach significantly reduces transmission cost while preserving high rendering quality and strong segmentation performance.

==> sec/method/compression_overview.tex <==
\begin{figure}[t]
    \centering
    \resizebox{\linewidth}{!}{
    \includegraphics[width=0.5\textwidth]{Figures/Overview&teaser/Compress_Overall.png}  
    }
    \caption{System Overview of our compression framework.}
    \label{fig:compress_overview}
\end{figure}



==> sec/related_work/Comparison_table.tex <==
% \begin{table}[t]
% \caption{Comparative analysis of Dynamic 3DGS approaches.}
% \label{tab:method_compare_table}
% \vspace{-0.5em}
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{l|ccc}
% \hline
% \textbf{Model} & \textbf{Temporal Activation}& \textbf{RD Comp.}& \textbf{Motion Modeling}\\
% \hline
% % DyNeRF         & 29.58 & 0.980 & 0.083                  & 0.015 & 28 \\
% % NeRFPlayer     & 30.69 & 0.966 & 0.111                  & 0.045 & -- \\
% % HexPlane       & 31.70 &0.987 & 0.075   & 0.2   & 250 \\
% % Mixvoxels      & 31.73 & --    & 0.064                  & 4.6   & 500 \\
% % HyperReel      & 31.10 & 0.964 & 0.096                  & 2.0   & 360 \\
% % \hline
% \multicolumn{4}{l}{\textbf{Space-time 4DGS}}\\   % <-- 新增的橫跨 4 欄列
% \hline
% 4DGS~\cite{yang2024realtimephotorealisticdynamicscene}  & \checkmark
% & $\times$ & Linear\\
% STG~\cite{li2024spacetimegaussianfeaturesplatting}            & $\checkmark$& $\times$ & Polynomial\\
%  4DScaffoldGS~\cite{cho20244dscaffoldgaussiansplatting}& $\checkmark$&$\times$ &Linear\\
% FreeTimeGS~\cite{wang2025freetimegsfreegaussianprimitives}     & $\checkmark$&$\times$ &  Linear\\
% \hline 
% \multicolumn{4}{l}{\textbf{Canonical 3DGS + Deformation}}\\   % <-- 新增的橫跨 4 欄列
% \hline
% % 3DGStream      & 31.67 & --    & --                     & 215 & 2340 \\
% % DN-4DGS        & 32.02 & 0.984 & 0.043 & 15    & 112 \\
% 4DGaussians~\cite{wu20244dgaussiansplattingrealtime}     &$\times$ &$\times$ & Coord.-based\\
% E-D3DGS~\cite{bae2024pergaussianembeddingbaseddeformationdeformable}        & $\times$&$\times$ & Embedding-based\\
% Light4GS~\cite{liu2025light4gslightweightcompact4d}&$\times$ & $\checkmark$& Coord.-based\\
% ADC-GS~\cite{huang2025adcgsanchordrivendeformablecompressed}& $\times$& $\checkmark$& Embedding-based\\
% \hline              
% Ours (TED-4DGS)& $\checkmark$& $\checkmark$  &Embedding-based\\
% \hline
% \end{tabular}
% }
% \end{table}

\begin{table}[t]
\caption{Comparative analysis of dynamic 3DGS approaches.}
\label{tab:method_compare_table}
\vspace{-0.6em}
\centering
\setlength{\tabcolsep}{2pt}   % 全域欄間距稍微小一點
\renewcommand{\arraystretch}{1.0}
\footnotesize

\begin{tabular}{@{} >{\raggedright\arraybackslash}p{2.2cm}
    !{\hspace{1pt}\vrule width 0.4pt\hspace{2pt}} % 自訂直線與兩側間距
    c c c @{}}
\hline
\textbf{Model} & \textbf{Temporal Activation} & \textbf{RD Comp.} & \textbf{Motion Model}\\
\hline
\multicolumn{4}{@{}l}{\textbf{Space-time 4DGS}}\\
\hline
4DGS~\cite{yang2024realtimephotorealisticdynamicscene} & \checkmark & $\times$ & Linear\\
STG~\cite{li2024spacetimegaussianfeaturesplatting}     & \checkmark & $\times$ & Polynomial\\
4DScaffoldGS~\cite{cho20244dscaffoldgaussiansplatting} & \checkmark & $\times$ & Linear\\
FreeTimeGS~\cite{wang2025freetimegsfreegaussianprimitives} & \checkmark & $\times$ & Linear\\
\hline
\noalign{\vskip 2pt} % 往下推下一行
\multicolumn{4}{l}{\shortstack[l]{\textbf{Canonical 3DGS }\\\textbf{+ Deformation}}}\\
\noalign{\vskip 1pt} % （可選）在它與下方 \hline 之間再加一點
\hline
4DGaussians~\cite{wu20244dgaussiansplattingrealtime} & $\times$ & $\times$ & Coord.-based\\
E-D3DGS~\cite{bae2024pergaussianembeddingbaseddeformationdeformable} & $\times$ & $\times$ & Embedding-based\\
Light4GS~\cite{liu2025light4gslightweightcompact4d} & $\times$ & \checkmark & Coord.-based\\
ADC-GS~\cite{huang2025adcgsanchordrivendeformablecompressed} & $\times$ & \checkmark & Embedding-based\\
\hline
Ours (TED-4DGS) & \checkmark & \checkmark & Embedding-based\\
\hline
\end{tabular}
\end{table}


==> sec/related_work/Taxonomy.tex <==
\begin{figure*}
  \centering
  \includegraphics[width=1\linewidth]{Figures/Overview&teaser/Dynamic_Taxonomy.png}
  \caption{Taxonomy of dynamic 3DGS representation.}
  \label{fig:taxonomy_dynamic3dgs}
\end{figure*}

